Reward Biased Maximum Likelihood Estimation for Reinforcement Learning

The Reward-Biased Maximum Likelihood Estimate (RBMLE) for adaptive control of Markov chains was proposed to overcome the central obstacle of what is variously called the fundamental "closed-identifiability problem" of adaptive control, the "dual control problem", or, contemporaneously, the "exploration vs. exploitation problem". It exploited the key observation that since the maximum likelihood parameter estimator can asymptotically identify the closed-transition probabilities under a certainty equivalent approach, the limiting parameter estimates must necessarily have an optimal reward that is less than the optimal reward attainable for the true but unknown system. Hence it proposed a counteracting reverse bias in favor of parameters with larger optimal rewards, providing a solution to the fundamental problem alluded to above. It thereby proposed an optimistic approach of favoring parameters with larger optimal rewards, now known as "optimism in the face of uncertainty". The RBMLE approach has been proved to be long-term average reward optimal in a variety of contexts. However, modern attention is focused on the much finer notion of "regret", or finite-time performance. Recent analysis of RBMLE for multi-armed stochastic bandits and linear contextual bandits has shown that it not only has state-of-the-art regret, but it also exhibits empirical performance comparable to or better than the best current contenders, and leads to strikingly simple index policies. Motivated by this, we examine the finite-time performance of RBMLE for reinforcement learning tasks that involve the general problem of optimal control of unknown Markov Decision Processes. We show that it has a regret of $\mathcal{O}( \log T)$ over a time horizon of $T$ steps, similar to state-of-the-art algorithms. Simulation studies show that RBMLE outperforms other algorithms such as UCRL2 and Thompson Sampling.

==> other_files/rebuttal_word_form.tex <==
We thank the reviewers for the valuable comments and suggestions that have helped us to greatly improve the paper. Below, we have tried our best to answer the concerns raised by the reviewers.

Response to Reviewer 1:

Constants in Theorem 9 are as follows:
\kappa_p is the conductivity of the underlying MDP, and loosely speaking measures how well the MDP "mixes" (for e.g. small kappa_p implies efficient exploration of different portions of the state-action space, and hence a lower regret). |X|, |U| are the cardinality of state and action spaces respectively. \Delta_{min} is the ''gap", i.e. the difference between rewards of optimal and second-best policy (its more difficult to estimate an optimal policy is gap is small, which in turn leads to a larger regret). 


Assumption 1 has been used in earlier works on reinforcement learning. For example "Optimal Adaptive Policies for Markov Decision Processes'', A.N. Burnetas and Michael N. Katehakis, Mathematics of Operations Research , Feb., 1997, Vol. 22, No. 1. This is in the same spirit (and equally hard to estimate whether or not it holds true) as other popularly used assumptions such as weakly communicating MDPs etc.

RBMLE is computationally simpler than UCB approaches (e.g. UCRL2). 

Response to Reviewer 2:

We believe that RBMLE went unnoticed by the Machine learning community (as was the case with Thompson sampling). Only recently has the community shown interest in RBMLE. Hence this work. In fact after our paper was submitted to L4DC, we performed extensive simulation results comparing RBMLE with Thompson Sampling and UCRL2. 

o(t) means that \lim_{t\to\infty} \frac{\alpha(t)}{t} =0.

As is discussed in the paper, considerable freedom is allowed while choosing f,\alpha(t). f can be any strictly monotone increasing function, and \alpha(t) must satisfy \alpha(t)=o(t),\lim_{t\to\infty}\alpha(t)=\infty.
